Mipha: A Comprehensive Overhaul of Multimodal Assistant with Small Language Models

Multimodal Large Language Models (MLLMs) have showcased impressive skills in tasks related to visual understanding and reasoning. Yet, their widespread application faces obstacles due to the high computational demands during both the training and inference phases, restricting their use to a limited audience within the research and user communities. In this paper, we investigate the design aspects of Multimodal Small Language Models (MSLMs) and propose an efficient multimodal assistant named Mipha, which is designed to create synergy among various aspects: visual representation, language models, and optimization strategies. We show that without increasing the volume of training data, our Mipha-3B outperforms the state-of-the-art large MLLMs, especially LLaVA-1.5-13B, on multiple benchmarks. Through detailed discussion, we provide insights and guidelines for developing strong MSLMs that rival the capabilities of MLLMs. Our code is available at https://github.com/zhuyiche/llava-phi.

==> qa_table.tex <==
\begin{table*}[tb]
  \centering
  \caption{Multi-modal evaluation on academic-task-oriented benchmarks. $\text{VQA}{\text{v2}}$~\cite{vqav2}; GQA~\cite{gqa}; VizWiz~\cite{vizwiz}; $\text{SQA}^{\text{I}}$: ScienceQA-IMG~\cite{scienceqa}; $\text{VQA}^{\text{T}}$: TextVQA~\cite{textvqa}. {$^*$}The training images/annotations of the datasets are observed during training. {$^ \dagger$} Includes in-house data that is not publicly accessible. Column \textit{Res.} is the image resolution of visual backbone. Columns \textit{PT} and \textit{IT} are the data sizes in the pretraining stage and the visual instruction tuning stage, respectively.}
  \label{tbl:qa_table}
  \resizebox{1.0\linewidth}{!}{
      \begin{tabular}{l|l|l|l|l|ccccc}
        \toprule
           Method & LLM  & Res. & PT & IT & $\text{VQAv2}$ &\text{GQA} &\text{VizWiz} & \text{SQA$^{\text{I}}$} & $\text{VQA}^{\text{T}}$  \\
        %\midrule
        %Gemini-Nano2~\cite{gemini} & N/A (3.25B)& - & - & 67.5 & - & - & 65.9 \\ 
        \midrule
        \multicolumn{10}{c}{Multimodal Large Language Models} \\
        \midrule
        %\textcolor{red}{OpenFlamingo}~\cite{openflamingo} & MBT (7B) & 336 & 180M & - & - & -& - & 33.6  \\
        BLIP-2~\cite{blip-2} & Vicuna (13B) & 224 & 129M & - & 65.0 & 41.0 & 19.6 & 61.0 & 42.5 \\
        InstructBLIP~\cite{instructblip} & Vicuna (7B) & 224 & 129M & 1.2M & - & 49.2 & 34.5 & 60.5 & 50.1  \\
        InstructBLIP~\cite{instructblip} & Vicuna (13B) & 224 & 129M & 1.2M & - & 49.5 & 33.4 & 63.1 & 50.7\\
        %\textcolor{red}{MiniGPT-4}~\cite{minigpt4} & Vicuna (7B) & - & - & - & - \\
        Shikra~\cite{shikra} & Vicuna (13B) & 224 & 600K & 5.5M &  77.4{$^*$} & - & - & - & - \\
        %\textcolor{red}{Otter}~\cite{otter} & LLaMA (7B) & - & - & - & -  \\
        IDEFICS-9B~\cite{idefics} & LLaMA (7B) & 224 & 353M & 1M & 50.9 & 38.4 & 35.5 & - & 25.9  \\
        IDEFICS-80B~\cite{idefics} & LLaMA (65B) & 224 & 353M & 1M & 60.0 & 45.2 & 36.0 & - & 30.9 \\
        Qwen-VL~\cite{qwen} & Qwen (7B) & 448 & 1.4B{$^\dagger$} & 50M{$^\dagger$} & 78.8{$^*$} & 59.3{$^*$} & 35.2 & 67.1 & \textbf{63.8}{$^*$} \\
        Qwen-VL-Chat~\cite{qwen} & Qwen (7B) & 448 & 1.4B{$^\dagger$} & 50M{$^\dagger$} & 78.2{$^*$} & 57.5{$^*$} & 38.9 & 68.2 & 61.5{$^*$} \\
        mPLUG-Owl2~\cite{mplugowl2} & LLaMA (7B) & 448 & 400M & 1.23M & 79.4 & 56.1 & \textbf{54.5} & 68.7 & 58.2 \\
        %\textcolor{red}{LLaVA}~\cite{llava} & Vicuna (7B) & - & - & - & -  \\
        LLaVA-1.5~\cite{llava1.5} & Vicuna (7B) & 336 & 558K & 665K  & 78.5{$^*$} & 62.0{$^*$} & 50.0 & 66.8 & 58.2  \\
        LLaVA-1.5~\cite{llava1.5} & Vicuna (13B) & 336 & 558K & 665K  & 80.0{$^*$} & 63.3{$^*$} & 53.6 & \textbf{71.6} & 61.3  \\
        \midrule
        \multicolumn{10}{c}{Multimodal Small Language Models} \\
        \midrule
        MobileVLM~\cite{chu2023mobilevlm} & M-LLaMA (2.7B) & 336 & 558K & 665K & - & 59.0 & - & 61.2 & 47.5 \\
        MobileVLM-v2~\cite{mobilevlmv2} & M-LLaMA (2.7B) & 336 & 1.2M & 2.4M & -  & 61.1 & - & 70.0 & 57.5  \\
        MoE-LLaVA-3.6B~\cite{moe-llava} & Phi-2 (2.7B) & 384 & 558k & 1.59M & 79.9{$^*$} & 62.6{$^*$} & 43.7 & 70.3 & 57.0 \\
        Bunny-3B~\cite{bunny} & Phi-2 (2.7B) & 384 & 2M & 695K & 79.8 & 62.5 & - & 70.9 & - \\
        \midrule
        Mipha-3B (Ours) & Phi-2 (2.7B)  & 384 & 558K & 665K & \textbf{81.3}{$^*$} & \textbf{63.9}{$^*$} & 47.5  & 70.9 & 56.6 \\
        \bottomrule
      \end{tabular}
    }
\end{table*}


